Geometric Median Matching for Robust k-Subset Selection from Noisy Data

Data pruning -- the combinatorial task of selecting a small and representative subset from a large dataset, is crucial for mitigating the enormous computational costs associated with training data-hungry modern deep learning models at scale. Since large scale data collections are invariably noisy, developing data pruning strategies that remain robust even in the presence of corruption is critical in practice. However, existing data pruning methods often fail under high corruption rates due to their reliance on empirical mean estimation, which is highly sensitive to outliers. In response, we propose Geometric Median (GM) Matching, a novel k-subset selection strategy that leverages Geometric Median -- a robust estimator with an optimal breakdown point of 1/2; to enhance resilience against noisy data. Our method iteratively selects a k-subset such that the mean of the subset approximates the GM of the (potentially) noisy dataset, ensuring robustness even under arbitrary corruption. We provide theoretical guarantees, showing that GM Matching enjoys an improved O(1/k) convergence rate -- a quadratic improvement over random sampling, even under arbitrary corruption. Extensive experiments across image classification and image generation tasks demonstrate that GM Matching consistently outperforms existing pruning approaches, particularly in high-corruption settings and at high pruning rates; making it a strong baseline for robust data pruning.

==> app-plots/gm/comp_time.tex <==
\begin{figure} 
\centering
\includegraphics[width=0.7\textwidth]{plots/weiszfeld/gm_wall_time.pdf}

\caption{ \footnotesize {\bf \textsc{Scaling Laws (Wall Clock) for $\gm$ Computation}}: 
This figure shows the scaling behavior for computing the geometric median using Weiszfeld algorithm (~\cref{algo:weiszfeld}) in terms of the wall clock time (\( T_{GM} \)) as a function of population size. The x-axis represents the number of samples (\( n \)) on a logarithmic scale, and the y-axis shows the average wall clock time (\( T_{GM} \)) on a logarithmic scale. Each curve corresponds to a different embedding dimension (\( d \)), ranging from 32 to 4096. The results were generated using synthetic data drawn from a standard normal distribution, with the geometric median computed iteratively until convergence (tolerance \( \epsilon = 10^{-5} \), maximum iterations = 100). For each combination of \( n \) and \( s \), wall clock time was averaged across 10 random seed. The computational cost increases with both \( n \) and \( s \): for fixed \( n \), the scaling with \( s \) is approximately linear, while for fixed \( s \), scaling with \( n \) exhibits sub-linear to near-linear growth. These results emphasize the trade-offs in selecting \( n \) and \( s \) for practical applications. Experiments were run on a single-threaded CPU setup. These results confirm that the practical runtime aligns with the expected time complexity of $\gO(ns\log(1/\epsilon))$ in typical scenarios, showcasing the efficiency of Weiszfeld algorithm for high-dimensional data.
}
\label{fig:app-comp-gm}
\end{figure}

==> app-plots/gmm/comp_time.tex <==
\begin{figure} 
\centering
\includegraphics[width=0.7\textwidth]{plots/toy/anisotropic/conv-batch/clean-bs_gmm_time.pdf}
\caption{ \footnotesize {\bf \textsc{Scaling Laws (Wall Clock) for Batch $\gmm$}} as a function of coreset size (k) across varying batch sizes (b). Log-log scale highlights the computational cost trends for batch sizes ranging from 1 to 1024.
}
\label{fig:app-comp-gmm}
\end{figure}

==> combined_table.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{cc}
            % First table
            \begin{tabular}{lcccc}
                \toprule
                & \multicolumn{2}{c}{\bf CIFAR-100 (PGD Attack)} & \multicolumn{2}{c}{\bf CIFAR-100 (GS Attack)} \\
                \cmidrule(r){2-3} \cmidrule(r){4-5}
                {\bf Method / Ratio } & 20\% & 30\% & 20\% & 30\% \\
                \midrule
                Random & 43.23$\pm$0.31 & 52.86$\pm$0.34 & 44.23$\pm$0.41 & 53.44$\pm$0.44 \\
                Herding & 40.21$\pm$0.72 & 49.62$\pm$0.65 & 39.92$\pm$1.03 & 50.14$\pm$0.15 \\
                Forgetting & 35.90$\pm$1.30 & 47.37$\pm$0.99 & 37.55$\pm$0.53 & 46.88$\pm$1.91 \\
                GraNd-score & 40.87$\pm$0.84 & 50.13$\pm$0.30 & 40.77$\pm$1.11 & 49.88$\pm$0.83 \\
                EL2N-score & 26.61$\pm$0.58 & 34.50$\pm$1.02 & 26.72$\pm$0.66 & 35.55$\pm$1.30 \\
                Optimization-based & 38.29$\pm$1.77 & 46.25$\pm$1.82 & 41.36$\pm$0.92 & 49.10$\pm$0.81 \\
                Self-sup.-selection & 40.53$\pm$1.15 & 49.95$\pm$0.50 & 40.74$\pm$1.66 & 51.23$\pm$0.25 \\
                Moderate-DS & 43.60$\pm$0.97 & 51.66$\pm$0.39 & 44.69$\pm$0.68 & 53.71$\pm$0.37 \\
                {\bf $\gm$ Matching} & {\bf 45.41$\pm$0.86} & {\bf 51.80$\pm$1.01} & {\bf 49.78$\pm$0.27} & {\bf 55.50$\pm$0.31} \\
                \bottomrule
            \end{tabular}
            &
            % Second table
            \begin{tabular}{lcccc}
                \toprule
                & \multicolumn{2}{c}{\bf CIFAR-100 (Label noise)} & \multicolumn{2}{c}{\bf Tiny ImageNet (Label noise)} \\
                \cmidrule(r){2-3} \cmidrule(r){4-5}
                {\bf Method / Ratio } & 20\% & 30\% & 20\% & 30\% \\
                \midrule
                Random & 34.47$\pm$0.64 & 43.26$\pm$1.21 & 17.78$\pm$0.44 & 23.88$\pm$0.42 \\
                Herding & 42.29$\pm$1.75 & 50.52$\pm$3.38 & 18.98$\pm$0.44 & 24.23$\pm$0.29 \\
                Forgetting & 36.53$\pm$1.11 & 45.78$\pm$1.04 & 13.20$\pm$0.38 & 21.79$\pm$0.43 \\
                GraNd-score & 31.72$\pm$0.67 & 42.80$\pm$0.30 & 18.28$\pm$0.32 & 23.72$\pm$0.18 \\
                EL2N-score & 29.82$\pm$1.19 & 33.62$\pm$2.35 & 13.93$\pm$0.69 & 18.57$\pm$0.31 \\
                Optimization-based & 32.79$\pm$0.62 & 41.80$\pm$1.14 & 14.77$\pm$0.95 & 22.52$\pm$0.77 \\
                Self-sup.-selection & 31.08$\pm$0.78 & 41.87$\pm$0.63 & 15.10$\pm$0.73 & 21.01$\pm$0.36 \\
                Moderate-DS & 40.25$\pm$0.12 & 48.53$\pm$1.60 & 19.64$\pm$0.40 & 24.96$\pm$0.30 \\
                {\bf $\gm$ Matching} & {\bf 52.64$\pm$0.72} & {\bf 61.01$\pm$0.47} & {\bf 25.80$\pm$0.37} & {\bf 31.71$\pm$0.24} \\
                \bottomrule
            \end{tabular}
        \end{tabular}
    }
    \caption{
        \footnotesize
         {\bf (Left) \textsc{(Label Noise) Image Classification:}} Comparing (Test Accuracy) pruning methods on CIFAR-100 and TinyImageNet datasets, under 20\% and 35\% Symmetric Label Corruption, at 20\% and 30\% selection ratio. ResNet-50 is used both as proxy and for downstream classification.
        Side-by-side comparison of (Test Accuracy) pruning methods under adversarial attacks (left) and label noise (right) across CIFAR-100 and Tiny ImageNet datasets. ResNet-50 is used both as proxy and for downstream classification. 
        {\bf (Right) \textsc{(Adversarial Attack) Image Classification:}} . Comparing (Test Accuracy) pruning methods under PGD and GS attacks. ResNet-50 is used both as proxy and for downstream classification.
    }
    \label{tab:combined}
\end{table*}

==> main-plots/fig-gm-conv.tex <==
\begin{figure}
\centering
\includegraphics[width=0.35\textwidth]{plots/toy/anisotropic/conv-estimation/conv_bs_gm.pdf} 
\includegraphics[width=0.7\textwidth]{plots/toy/anisotropic/conv-batch/clean-bs_gmm_time.pdf}
\caption{
\footnotesize 
{\bf \textsc{Gm Scaling (Convergence)}:}
Comparison of Mean Estimation Error i.e. deviation of $\gm$ from the oracle mean $\|\Mu_\epsilon^\gm - \Mu_\gG\|^2$ w.r.t sample size $|\gD|$ and corruption rate $\psi$.
}
\label{fig:main-conv-gm}
\end{figure}

==> main-plots/fig-gm-wall.tex <==
\begin{figure}[htb!] 
\centering
\includegraphics[width=0.4\textwidth]{plots/weiszfeld/gm_wall_time.pdf}
\caption{
\footnotesize 
{\bf \textsc{Gm Scaling (Convergence)}:}
}
\label{fig:main-wall-gm}
\end{figure}

==> plots/diffusion/mnist/corruption_types/clip-pca/fig.tex <==
\begin{figure}[htbp]
    \centering
    % First row of subfigures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/diffusion/mnist/corruption_types/clip-pca/clean.png}
        \caption{Clean Samples}
    \end{subfigure}    
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/diffusion/mnist/corruption_types/clip-pca/gaussian.png}
        \caption{(Additive) Gaussian Noise}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/diffusion/mnist/corruption_types/clip-pca/uniform.png}
        \caption{(Additive) Uniform Noise}
    \end{subfigure}

    \vspace{1.5em}
    
    % Second row of subfigures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/diffusion/mnist/corruption_types/clip-pca/random_patches.png}
        \caption{Random Patches}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/diffusion/mnist/corruption_types/clip-pca/cutout.png}
        \caption{Cutout Noise}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/diffusion/mnist/corruption_types/clip-pca/random_image.png}
        \caption{Random Noise}
    \end{subfigure}

    \caption{{\bf (PCA)} Visualization of CLIP ViT-B/32 Embeddings of a subset of MNIST images :  
    (a) Clean (baseline), and where 45\% samples corrupted with (b) Gaussian noise, (c) Uniform noise, (d) Random patches, (e) Cutout noise.}
    \label{fig:diffusion_noise_samples_pca_mnist}
\end{figure}



==> plots/toy/anisotropic/moments/fig.tex <==
\begin{figure*}[htb!] 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[{\bf No Corruption} ($\psi = 0$)]{
\includegraphics[width=0.32\textwidth]{plots/toy/anisotropic/moments/corr=0.pdf}}
\subfloat[{\bf 20\% Corruption} ($\psi = 0.2$)]
{\includegraphics[width=0.32\textwidth]{plots/toy/anisotropic/moments/corr=0.2.pdf}}
\subfloat[{\bf 40\% Corruption} ($\psi = 0.4$)]
{\includegraphics[width=0.32\textwidth]{plots/toy/anisotropic/moments/corr=0.4.pdf}}

\caption{
\footnotesize {
\bf \textsc{Robust Mean Estimation}}: 
This figure illustrates the deviation of the Empirical Mean (\textcolor{red}{red}) and Geometric Median (\textcolor{purple}{purple}) from the Oracle Mean (\textcolor{teal}{green}) as the fraction of corrupted samples $0 \leq \psi < 1/2$ is varied. The uncorrupted distribution is shown in \textcolor{blue}{\bf Blue}, while the adversarial distribution is shown in \textcolor{red}{red}. At \(\psi = 0\), all estimators align closely with the oracle mean. As \(\psi\) increases, the empirical mean is significantly influenced by the corrupted samples, drifting toward the corrupted distribution. In contrast, the $\gm$ remains robust, staying closer to the oracle mean demonstrating the resilience of the $\gm$ in the presence of corruptions.
}
\label{fig:app-toy-moment}
\end{figure*}

==> plots/toy/fig.toy-all.tex <==
\begin{figure} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[Uniform ($\psi=0$)]{
\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/uniform.png}}
\subfloat[Uniform ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/uniform.png}}
\subfloat[Uniform ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/uniform.png}}
\\
\subfloat[Easy ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/easy.png}}
\subfloat[Easy ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/easy.png}}
\subfloat[Easy ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/easy.png}}
\\
\subfloat[Hard ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/hard.png}}
\subfloat[Hard ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/hard.png}}
\subfloat[Hard ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/hard.png}}
\\
\subfloat[Moderate ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/moderate.png}}
\subfloat[Moderate ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/moderate.png}}
\subfloat[Moderate ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/moderate.png}}
\\
\subfloat[Herding ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/herding.png}}
\subfloat[Herding ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/herding.png}}
\subfloat[Herding ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/herding.png}}
\\
\subfloat[Robust Herding ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/robust-herding.png}}
\subfloat[Robust Herding ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/robust-herding.png}}
\subfloat[Robust Herding ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/robust-herding.png}}
\caption{\footnotesize Toy Example.}

\label{fig:toy-allcorr=45}
\end{figure}

==> plots/toy/fig.toy-corr=0.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*}[t] 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[Random]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=0/uniform.png}}
\subfloat[Easy]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=0/easy.png}}
\subfloat[Hard]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=0/hard.png}}
\\
\subfloat[Moderate]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=0/moderate.png}}
\subfloat[Herding]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=0/herding.png}}
\subfloat[$\gmm$]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=0/robust-herding.png}}
\caption{\footnotesize 
{\bf \textsc{(Sampling from Gaussian) No Corruption ($\psi=0$) :} 
} We subset 10\% of the samples using baseline subset selection strategies: Uniform, Easy, Hard, Moderate, Kernel Herding, \textsc{GM Matching} (\cref{sec:exp-baselines}). $\gmm$ and Kernel Herding use identity kernel map $\phi(\vx) = \vx$. 
}
\label{fig:exp-syn-corr=0}
\end{figure*}

==> plots/toy/fig.toy-corr=20.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*}[t]
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[Random]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=20/uniform.png}}
\subfloat[Easy]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=20/easy.png}}
\subfloat[Hard]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=20/hard.png}}
\\
\subfloat[Moderate]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=20/moderate.png}}
\subfloat[Kernel Herding]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=20/herding.png}}
\subfloat[$\gmm$]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=20/robust-herding.png}}
\caption{\footnotesize {\bf \textsc{(Sampling from Noisy Gaussian) 20\% Corruption ($\psi=0.2$)}}: In this experiment, 20\% of the samples are corrupted -- drawn from a adversary chosen distribution (red). We select 10\% samples baseline subset selection strategies: Uniform, Easy, Hard, Moderate, Kernel Herding, \textsc{GM Matching} (\cref{sec:exp-baselines}). $\gmm$ and Kernel Herding are performed using an identity kernel map $\phi(\vx) = \vx$. We see that while Easy remains robust, it is clearly sampling from low-density areas -- failing to capture the prototypical samples.}
\label{fig:exp-syn-corr=20}
\end{figure*}

==> plots/toy/fig.toy-corr=45.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*}[t] 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[Random]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=45/uniform.png}}
\subfloat[Easy]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=45/easy.png}}
\subfloat[Hard]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=45/hard.png}}
\\
\subfloat[Moderate]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=45/moderate.png}}
\subfloat[Herding]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=45/herding.png}}
\subfloat[$\gmm$]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=45/robust-herding.png}}
\caption{\footnotesize {\bf \textsc{(Sampling from Noisy Gaussian)45\% Corruption ($\psi=0.45$)}} i.e. drawn from an adversary chosen distribution (red). We compare several baselines for choosing 10\% samples: Uniform, Easy, Hard, Moderate, Kernel Herding, \textsc{GM Matching} (\cref{sec:exp-baselines}). $\gmm$ and Kernel Herding are performed using an identity kernel map $\phi(\vx) = \vx$. Clearly $\gmm$ is significantly more robust and diverse than the other approaches even at such high corruption rates.}

\label{fig:exp-syn-corr=45}
\end{figure*}

==> plots/toy/fig.toy-trade-off.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[\textsc{Easy ($\psi=0$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/easy.png}}
\subfloat[\textsc{Easy ($\psi=0.2$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/easy.png}}
\subfloat[\textsc{Easy ($\psi=0.45$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/easy.png}}
\\
\subfloat[\textsc{Hard ($\psi=0$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/hard.png}}
\subfloat[\textsc{Hard ($\psi=0.2$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/hard.png}}
\subfloat[\textsc{Hard ($\psi=0.45$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/hard.png}}
\\
\subfloat[\textsc{Gm Matching ($\psi=0$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/robust-herding.png}}
\subfloat[\textsc{Gm Matching ($\psi=0.2$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/robust-herding.png}}
\subfloat[\textsc{Gm Matching ($\psi=0.45$)}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/robust-herding.png}}
\\
\caption{\footnotesize {\bf Toy Example:} {\bf 0/20/45\% of the samples are corrupted} i.e. drawn from an adversary chosen distribution (red). We compare several baselines for choosing 10\% samples: (\textsc{Uniform}) random sampling, (\textsc{Easy}) selects of samples closest to the centroid. (\textsc{Hard}) Selection of samples farthest from the centroid. (\textsc{Moderate}) selects samples closest to the median distance from the centroid. (\textsc{Herding}) moment matching, (\textsc{GM Matching}) robust moment (GM) matching. Clearly $\gm$ Matching is significantly more robust and diverse than the other approaches even at such high corruption rates.}

\label{fig:toy-trade-off}
\end{figure*}

==> plots/weiszfeld/fig.tex <==
\begin{figure*} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[Mean Estimation Error]{
\includegraphics[width=0.32\textwidth]{plots/weiszfeld/gm_conv_bs.pdf}}
\subfloat[(Theoretical) Scaling Law]
{\includegraphics[width=0.32\textwidth]{plots/weiszfeld/gm_comp_theory.pdf}}
\subfloat[(Wall Clock) Scaling Law]
{\includegraphics[width=0.32\textwidth]{plots/weiszfeld/gm_wall_time.pdf}}
\caption{\footnotesize {\bf \textsc{Scaling Laws for $\gm$ Computation}}
}
\label{fig:comp-gm}
\end{figure*}

==> sections/theory.tex <==
% \input{main-plots/fig-scaling}
Notably, $\gmm$ is an infinite memory, deterministic process as at any iteration $t=T$, $\vtheta_T$ encapsulates the entire sampling history: 
\[
\vtheta_T = \vtheta_0 + T\Mu^\gm_\epsilon - \sum_{t=1}^T \phi(\vx_t)
\]
% \begin{equation}
%     \vtheta_T = \vtheta_0 + T\Mu^\gm_\epsilon - \sum_{t=1}^T \phi(\vx_t)
% \end{equation}
% $\vtheta_T = \vtheta_0 + T\Mu^\gm_\epsilon - \sum_{t=1}^T \phi(\vx_t)$. 
% Let, $\vtheta_0 = \Mu^\gm_\epsilon$, then, at each iteration $t=T$ $\gmm$ is performing the following greedy update:
% \[
% \vx_{T+1}=\argmax_{\vx \in \gD} \bigg[ \langle \Mu^\gm_\epsilon,\phi(\vx) \rangle - \frac{1}{T+1} \sum_{t=1}^T \omega(\vx, \vx_t)\bigg]
% \]
Conceptually, {\em $\vtheta_T$ represents the vector pointing towards under-sampled regions of the target distribution induced by $\gD$ at iteration $T$.}
% The algorithm's greedy selection strategy aligns each new sample with $\vtheta$, effectively {\em herding} new points to fill the gaps left by earlier selections. 
Greedy updates in the direction that reduces the accumulated error encourage the algorithm to explore underrepresented regions of the feature space, {\bf promoting diversity}. By matching the $\gm$ rather than the empirical mean, the algorithm imposes larger penalties on outliers, which lie farther from the core distribution,
% This encourages $\gmm$ to 
{\bf prioritizing samples near the convex hull of uncorrupted points} $\gC_\gG = \text{conv}\{\phi_\gB(\vx) | \vx \in \gD_\gG\}$. As a result, the algorithm promotes diversity in a balanced manner, effectively exploring different regions of the distribution while avoiding distant, noisy points, thus {\bf mitigating the robustness vs. diversity trade-off} discussed in \cref{sec:intro}. 

\input{plots/toy/anisotropic/conv-sampling/fig}

% \input{main-plots/fig-gm-conv}

{\bf \textsc{Convergence Guarantee}: }

In order to theoretically characterize the convergence behavior of $\gmm$, we first exploit the robustness property of $\gm$ to get an upper bound on the estimation error w.r.t the underlying oracle mean~\citep{pmlr-v151-acharya22a,chen2017distributed}. Next, we use the property that $\gm$ is guaranteed to lie in the interior of the convex hull of majority of the samples~\citep{boyd2004convex}. Combining these proof ideas we establish the following convergence guarantee:

\begin{theorem}
Suppose that we are given a set of grossly corrupted samples $\gD = \gD_\gG \cup \gD_\gB$ (\cref{def:corruption_model}), an $\epsilon$ approx. $\gm(\cdot)$ oracle~\eqref{eq:gm} and characteristic feature map $\phi(\cdot):\sR^d \to \gH$. Further assume that $\|\phi(\vx)\| \leq R \; \forall \vx \in \gD$ for some constant $R$. Then, $\gmm$ guarantees that the mean of the selected $k$-subset $\gD_\gS \subseteq \gD$ converges to a $\delta$-neighborhood of the uncorrupted (true) mean $\bm{\mu}^\gG = \E_{\vx \in \gD_\gG}(\phi(\vx))$ at the rate $\gO(1/k)$ such that:   
\begin{flalign}
\label{equation:bound-z0-simplified}
    \delta^2 \leq 
    \frac{8|\gD_\gG|^2}{(|\gD_\gG|-|\gD_\gB|)^2}\sigma^2_{\gG} + \frac{2\epsilon^2}{(|\gD_\gG|-|\gD_\gB|)^2}
\end{flalign}
where, 
$\sigma^2_{\gG} = \frac{1}{|\gD_\gG|}\sum_{\vx \in \gD_\gG}\E\|\phi(\vx) -\Mu^\gG\|^2$ denotes the variance of the uncorrupted samples.
\label{th:gm_match_cvg}
\end{theorem}
This result suggests that, even under gross corruption, $\gmm$ converges to a neighborhood of the true mean, where the neighborhood radius depends on two terms -- the first term depends on the variance of the uncorrupted samples and the second term depends on how accurately the $\gm$ is calculated. Furthermore, the bound holds $\forall \alpha = \gD_\gB / \gD_\gG < 1$ implying $\gm$ Matching remains robust even when $1/2$ of the samples are arbitrarily corrupted, i.e. it achieves the optimal breakdown point of 1/2. 
Furthermore, $\gmm$ achieves a convergence rate of $\gO(1/k)$ — a quadratic improvement over random sampling ($\gO(1/\sqrt{k})$). While Kernel Herding~\citep{chen2010super} also attains $\gO(1/k)$ in the clean setting, it deteriorates under noise, whereas $\gmm$ maintains this rate, as verified empirically in \cref{fig:main-toy-conv-mme}. \cref{sec:app-proof} contains the detailed proofs. 
% The convergence rate $\gO(1/k)$ is a quadratic improvement over random sampling which achieves $\gO(\frac{1}{\sqrt{k}})$. While Kernel Herding~\citep{chen2010super} achieves the same convergence rate in the clean setting --However, $\gmm$ is able to maintain this rate even in noisy setting -- where traditional kernel herding breaks down as verified empirically in \cref{fig:main-toy-conv-mme}.  
% \subsubsection*{Proof Outline}
% In order to theoretically characterize the convergence behavior of $\gmm$, we first exploit the robustness property of $\gm$ ~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed} to get an upper bound on the estimation error w.r.t the underlying true mean. 

% We can exploit the robustness property of $\gm$ to get an upper bound on the estimation error incurred by 
% show that the estimation error remains bounded w.r.t the underlying true mean~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed} even even in presence of grossly corrupted samples (unbounded). 
% % Intuitively, if such a subset can be found, the expected cost (e.g. loss / average gradient) over $\gS$ is guaranteed to be close (as characterized in~\cref{th:gm_match_cvg}) to the expected cost over the uncorrupted examples $\gD_\gG$; enabling robust data pruning. 

% This is because, even in presence of grossly corrupted samples (unbounded), $\gm$ remains bounded w.r.t the underlying true mean~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed}.

==> sections/warmup.tex <==
In the uncorrupted setting i.e. when $\gD_\gB = \emptyset$, a natural approach for data pruning is to formulate it as a combinatorial \textsc{moment matching} objective: 
\begin{equation}
    \argmin_{\gD_\gS \subseteq \gD, |\gD_\gS| = k}
    \bigg\| \frac{1}{|\gD|}\sum_{\vx_i \in \gD}\vx_i - \frac{1}{k} \sum_{\vx_i \in \gD_\gS}\vx_i\bigg\|^2
\label{eq:moment_matching}
\end{equation}
Needless to say, identifying sample importance is an ill-posed problem without some notion of similarity among the samples. Thus, it is common to assume access to a proxy encoder 
that maps the features to a separable embedding space. Intuitively, this simply means that the embedding space of the encoder fosters proximity of semantically similar examples, while enforcing the separation of dissimilar ones -- a property often satisfied by off-the-shelf pretrained foundation models~\citep{hessel2021clipscore, sorscher2022beyond, Radford2021LearningTV}.

Observe that,~\eqref{eq:moment_matching} is an instance of the famous set function maximization problem -- known to be NP-hard via a reduction from $k$-set cover~\citep{feige1998threshold}. Despite its intractability,~\citep{mirzasoleiman2020coresets} 
 demonstrated a transformation into a submodular set cover problem, enabling efficient solution via greedy algorithms~\citep{nemhauser1978analysis, wolsey1982analysis}. 
 
A popular greedy approach referred to as herding~\citep{welling2009herding, welling2010statistical} is to start with a suitably chosen $\boldsymbol{\theta}_0 \in \sR^d$; and iteratively adding samples via the following update rule:
\begin{flalign}
\vx_{t+1} &:= \argmax_{\vx \in \gD} \; \langle\vtheta_t, \vx\rangle
\label{eq:samle_update_mean}
\\
\vtheta_{t+1} 
&:= \vtheta_t + \bigg( \frac{1}{|\gD|}\sum_{\vx_i \in \gD}\vx_i - \vx_{t+1} \bigg)
\label{eq:theta_update_mean}
\end{flalign}
It's worth noting that this algorithm is an infinite memory, deterministic process as at each iteration T, $\vtheta_T$ encapsulates the entire sampling history: $\vtheta_T = \vtheta_0 + T\bm{\mu} - \sum_{t=1}^T \vx_t$ where $\bm{\mu} = \frac{1}{|\gD|}\sum_{\vx_i \in \gD}\vx_i$. Conceptually, $\vtheta_T$ represents the vector pointing towards under-sampled regions of the target distribution induced by $\gD$ at iteration $T$. Remarkably,~\citep{chen2010super} showed that this simple greedy update rule achieves an impressive $\gO(1/k)$ convergence rate for~\eqref{eq:moment_matching}, a quadratic improvement over random sampling where the error decreases at the rate $\gO(1/\sqrt{k})$. The result holds if $\|\vx\| \leq R \; \forall \vx \in \gD$ for some constant $R$ and as long as the target moment is in the relative interior of $\gC = \text{conv}\{\vx | \vx \in \gD\}$ (Proposition 1~\citep{chen2010super}).

% \subsubsection*{Vulnerability Under Corruption}
% Despite its strong performance guarantees in the vanilla (uncorrupted) setting, we argue that the algorithm can result in arbitrarily poor solution in the noisy setting. The vulnerability can be attributed to the estimation of target moment via empirical mean -- notorious for its sensitivity to outliers. Consider a single adversarial sample: $\vx^\gB = |\gD|\bm{\mu}^\gB - \sum_{\vx \in \gD\setminus\vx^\gB}\vx$, shifting the empirical mean to adversary chosen arbitrary target $\bm{\mu}^\gB$. This implies that the empirical mean can't tolerate even a single grossly corrupted sample i.e. yields {\bf lowest possible asymptotic breakdown point of 0}. As a consequence, optimizing over the moment matching objective~\eqref{eq:moment_matching} no longer guarantee convergence to the true underlying (uncorrupted) moment, instead the algorithm can be hijacked by a single bad sample, warping the solution toward an adversarial target.   


==> tables/benchmark/tab-clean-net-transfer.tex <==
\begin{table*}
    \footnotesize
    \centering
    \begin{tabular}{lccccc}
        \toprule
        
        & \multicolumn{2}{c}{\bf ResNet-50→SENet}
        & \multicolumn{2}{c}{\bf ResNet-50→EfficientNet-B0} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf Mean $\uparrow$} 
        \\
        \midrule
        Random 
        & 34.13$\pm$0.71 
        & 39.57$\pm$0.53 
        & 32.88$\pm$1.52 
        & 39.11$\pm$0.94 
        & 36.42 
        \\ 
        Herding 
        & 34.86$\pm$0.55 
        & 38.60$\pm$0.68 
        & 32.21$\pm$1.54 
        & 37.53$\pm$0.22 
        & 35.80
        \\
        Forgetting 
        & 33.40$\pm$0.64 
        & 39.79$\pm$0.78 
        & 31.12$\pm$0.21 
        & 38.38$\pm$0.65 
        &  35.67
        \\
        GraNd-score 
        & 35.12$\pm$0.54 
        & 41.14$\pm$0.42 
        & 33.20$\pm$0.67 
        & 40.02$\pm$0.35
        & 37.37
        \\
        EL2N-score 
        & 31.08$\pm$1.11 
        & 38.26$\pm$0.45 
        & 31.34$\pm$0.49 
        & 36.88$\pm$0.32 
        & 34.39
        \\
        Optimization-based 
        & 33.18$\pm$0.52 
        & 39.42$\pm$0.77 
        & 32.16$\pm$0.90 
        & 38.52$\pm$0.50 
        & 35.82
        \\
        Self-sup.-selection 
        & 31.74$\pm$0.71 
        & 38.45$\pm$0.39 
        & 30.99$\pm$1.03 
        & 37.96$\pm$0.77 
        & 34.79
        \\
        Moderate-DS 
        & 36.04$\pm$0.15
        & 41.40$\pm$0.20 
        & 34.26$\pm$0.48 
        & 39.57$\pm$0.29 
        & 37.82
        \\
        {\bf $\gm$ Matching} 
        & {\bf 37.93$\pm$0.23} 
        & {\bf 42.59$\pm$0.29}
        & {\bf 36.31$\pm$0.67}
        & {\bf 41.03$\pm$0.41} 
        & {\bf 39.47}
        \\
        \bottomrule
    \end{tabular}
    \caption
    {
    \footnotesize
    {\bf Network Transfer (Clean)} : Tiny-ImageNet Model Transfer Results. A ResNet-50 proxy is used to find important samples which are then used to train SENet and EfficientNet.
    }
    \label{tab:clean-nw-transfer}
\end{table*}


==> tables/benchmark/tab-clean.tex <==
\begin{table*}
\footnotesize
\centering
\resizebox{\textwidth}{!}
{
    \begin{tabular}{lccccccc}
        \midrule
        \rowcolor{light-gray}
        \multicolumn{8}{c}{{\bf CIFAR-100}}
        \\
        \midrule
        {\textbf{Method / Ratio}} 
        & \textbf{20\%} 
        & \textbf{30\%} 
        & \textbf{40\%}
        & \textbf{60\%}
        & \textbf{80\%}
        & \textbf{100\%}
        & \textbf{Mean $\uparrow$}
        \\ 
        \midrule
        Random              
        & 50.26$\pm$3.24 
        & 53.61$\pm$2.73 
        & 64.32$\pm$1.77 
        & 71.03$\pm$0.75 
        & 74.12$\pm$0.56 
        & 78.14$\pm$0.55 
        & 62.67
        \\ 
        Herding               
        & 48.39$\pm$1.42 
        & 50.89$\pm$0.97 
        & 62.99$\pm$0.61 
        & 70.61$\pm$0.44 
        & 74.21$\pm$0.49 
        & 78.14$\pm$0.55 
        & 61.42
        \\ 
        Forgetting            
        & 35.57$\pm$1.40 
        & 49.83$\pm$0.91 
        & 59.65$\pm$2.50 
        & \textbf{73.34$\pm$0.39} 
        & \textbf{77.50$\pm$0.53} 
        & 78.14$\pm$0.55 
        & 59.18
        \\ 
        GraNd-score           
        & 42.65$\pm$1.39 
        & 53.14$\pm$1.28 
        & 60.52$\pm$0.79 
        & 69.70$\pm$0.68 
        & 74.67$\pm$0.79 
        & 78.14$\pm$0.55
        & 60.14
        \\ 
        EL2N-score            
        & 27.32$\pm$1.16 
        & 41.98$\pm$0.54 
        & 50.47$\pm$1.20 
        & 69.23$\pm$1.00 
        & 75.96$\pm$0.88 
        & 78.14$\pm$0.55
        & 52.99
        \\ 
        Optimization-based    
        & 42.16$\pm$3.30 
        & 53.19$\pm$2.14 
        & 58.93$\pm$0.98 
        & 68.93$\pm$0.70 
        & 75.62$\pm$0.33 
        & 78.14$\pm$0.55 
        & 59.77
        \\
        Self-sup.-selection   
        & 44.45$\pm$2.51
        & 54.63$\pm$2.10 
        & 62.91$\pm$1.20 
        & 70.70$\pm$0.82 
        & 75.29$\pm$0.45 
        & 78.14$\pm$0.55 
        & 61.60
        \\ 
        Moderate-DS
        & 51.83$\pm$0.52
        & 57.79$\pm$1.61
        & 64.92$\pm$0.93
        & 71.87$\pm$0.91 
        & 75.44$\pm$0.40 
        & 78.14$\pm$0.55 
        & 64.37
        \\ 
        {\bf $\gm$ Matching}  
        & {\bf 55.93$\pm$ 0.48}
        & {\bf 63.08$\pm$ 0.57}
        & {\bf 66.59$\pm$ 1.18} 
        & 70.82$\pm$ 0.59
        & 74.63$\pm$ 0.86
        & 78.14$\pm$ 0.55  
        & {\bf 66.01}
        \\
        \midrule
        \rowcolor{light-gray}
        \multicolumn{8}{c}{{\bf Tiny ImageNet}}
        \\
        \midrule
        Random              
        & 24.02$\pm$0.41 
        & 29.79$\pm$0.27 
        & 34.41$\pm$0.46 
        & 40.96$\pm$0.47 
        & 45.74$\pm$0.61 
        & 49.36$\pm$0.25 
        & 34.98 
        \\ 
        Herding               
        & 24.09$\pm$0.45 
        & 29.39$\pm$0.53 
        & 34.13$\pm$0.37 
        & 40.86$\pm$0.61 
        & 45.45$\pm$0.33 
        & 49.36$\pm$0.25 
        & 34.78 
        \\ 
        Forgetting            
        & 22.37$\pm$0.71 
        & 28.67$\pm$0.54 
        & 33.64$\pm$0.32 
        & 41.14$\pm$0.43 
        & \textbf{46.77$\pm$0.31} 
        & 49.36$\pm$0.25 
        & 34.52
        \\ 
        GraNd-score           
        & 23.56$\pm$0.52 
        & 29.66$\pm$0.37 
        & 34.33$\pm$0.50 
        & 40.77$\pm$0.42 
        & 45.96$\pm$0.56 
        & 49.36$\pm$0.25 
        & 34.86 
        \\ 
        EL2N-score            
        & 19.74$\pm$0.26 
        & 26.58$\pm$0.40 
        & 31.93$\pm$0.28 
        & 39.12$\pm$0.46 
        & 45.32$\pm$0.27 
        & 49.36$\pm$0.25 
        & 32.54
        \\ 
        Optimization-based    
        & 13.88$\pm$2.17 
        & 23.75$\pm$1.62 
        & 29.77$\pm$0.94 
        & 37.05$\pm$2.81 
        & 43.76$\pm$1.50 
        & 49.36$\pm$0.25 
        & 29.64
        \\
        Self-sup.-selection   
        & 20.89$\pm$0.42 
        & 27.66$\pm$0.50 
        & 32.50$\pm$0.30 
        & 39.64$\pm$0.39 
        & 44.94$\pm$0.34 
        & 49.36$\pm$0.25 
        & 33.13
        \\ 
        Moderate-DS
        & 25.29$\pm$0.38
        & 30.57$\pm$0.20
        & 34.81$\pm$0.51
        & 41.45$\pm$0.44
        & 46.06$\pm$0.33 
        & 49.36$\pm$0.25 
        & 35.64
        \\ 
        {\bf $\gm$ Matching}  
        & {\bf 27.88$\pm$0.19}
        & {\bf 33.15$\pm$0.26}
        & {\bf 36.92$\pm$0.40}
        & {\bf 42.48$\pm$0.12}
        & 46.75$\pm$0.51
        & 49.36$\pm$0.25 
        & {\bf 37.44}
        \\
        \bottomrule
    \end{tabular}
}
    \caption{
    \footnotesize
    {\bf No Corruption :} Comparing (Test Accuracy) pruning algorithms on CIFAR-100 and Tiny-ImageNet in the uncorrupted setting. ResNet-50 is used both as proxy and for downstream classification.}
    \label{tab:clean}
\end{table*}

==> tables/benchmark/tab-corrupt-30.tex <==
\begin{table*}
    \footnotesize
    \centering
    \resizebox{0.8\textwidth}{!}
    {
    \begin{tabular}{lccccc}
        \toprule
        \rowcolor{light-gray}
        \multicolumn{6}{c}{\bf 30\% Image Corruption}
        \\
        \midrule
        & \multicolumn{2}{c}{\bf CIFAR-100 } 
        & \multicolumn{2}{c}{\bf Tiny ImageNet} 
        & 
        \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio }
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf Mean $\uparrow$}
        \\
        \midrule
        Random 
        & 24.51$\pm$1.34 
        & 32.26$\pm$0.81 
        & 14.64$\pm$0.29 
        & 19.41$\pm$0.45 
        & 22.21
        \\
        Herding 
        & 29.42$\pm$1.54 
        & 37.50$\pm$2.12
        & 15.14$\pm$0.45 
        & 20.19$\pm$0.45 
        & 25.56
        \\
        Forgetting 
        & \textbf{29.48}$\pm$1.98 
        & \textbf{38.01}$\pm$2.21 
        & 11.25$\pm$0.90 
        & 17.07$\pm$0.66 
        & 23.45
        \\
        GraNd-score 
        & 23.03$\pm$1.05 
        & 34.83$\pm$2.01 
        & 13.68$\pm$0.46 
        & 19.51$\pm$0.45 
        & 22.26
        \\
        EL2N-score 
        & 21.95$\pm$1.08 
        & 31.63$\pm$2.84 
        & 10.11$\pm$0.25 
        & 13.69$\pm$0.32 
        & 19.34
        \\
        Optimization-based 
        & 26.77$\pm$0.15 
        & 35.63$\pm$0.92
        & 12.37$\pm$0.68 
        & 18.52$\pm$0.90 
        & 23.32
        \\
        Self-sup.-selection 
        & 23.12$\pm$1.47 
        & 34.85$\pm$0.68 
        & 11.23$\pm$0.32 
        & 17.76$\pm$0.69 
        & 21.74
        \\
        Moderate-DS 
        & 28.45$\pm$0.53 
        & 36.55$\pm$1.26 
        & {\bf 15.27$\pm$0.38 }
        & {\bf 20.33$\pm$0.28}
        & {\bf 25.65}
        \\
        {\bf $\gmm$} 
        & {\bf 42.28$\pm$1.02}
        & {\bf 54.71$\pm$0.86}
        & {\bf 23.38$\pm$1.09}
        & {\bf 27.93$\pm$0.98}
        & {\bf 37.08}
        \\
        \bottomrule
    \end{tabular}
    }
    \caption{
    \footnotesize
    {\bf \textsc{(Feature Corruption) Image Classification:}} Comparing (Test Accuracy) pruning methods on CIFAR-100 and TinyImageNet datasets, with 30\% corrupted data, at 20\% and 30\% selection ratio. ResNet-50 is used both as proxy and for downstream classification. Top 2 Best results in each column are highlighted.}
    \label{tab:corrupt-30}
\end{table*}


==> tables/benchmark/tab-main-A.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \resizebox{0.7\textwidth}{!}
{
    \begin{tabular}{lccccc}
        \toprule
        & \multicolumn{2}{c}{\bf CIFAR-100 (PGD Attack)} 
        & \multicolumn{2}{c}{\bf CIFAR-100 (GS Attack)} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & 20\% 
        & 30\% 
        & 20\% 
        & 30\% 
        & {\bf Mean $\uparrow$} 
        \\
        \midrule
        Random 
        & 43.23$\pm$0.31 
        & 52.86$\pm$0.34 
        & 44.23$\pm$0.41 
        & 53.44$\pm$0.44 
        & 48.44
        \\
        Herding 
        & 40.21$\pm$0.72 
        & 49.62$\pm$0.65 
        & 39.92$\pm$1.03 
        & 50.14$\pm$0.15 
        & 44.97
        \\
        Forgetting 
        & 35.90$\pm$1.30 
        & 47.37$\pm$0.99 
        & 37.55$\pm$0.53 
        & 46.88$\pm$1.91 
        & 41.93
        \\
        GraNd-score 
        & 40.87$\pm$0.84 
        & 50.13$\pm$0.30 
        & 40.77$\pm$1.11 
        & 49.88$\pm$0.83 
        & 45.41
        \\
        EL2N-score 
        & 26.61$\pm$0.58 
        & 34.50$\pm$1.02 
        & 26.72$\pm$0.66 
        & 35.55$\pm$1.30 
        & 30.85
        \\
        Optimization-based 
        & 38.29$\pm$1.77 
        & 46.25$\pm$1.82 
        & 41.36$\pm$0.92 
        & 49.10$\pm$0.81 
        & 43.75
        \\
        Self-sup.-selection 
        & 40.53$\pm$1.15 
        & 49.95$\pm$0.50 
        & 40.74$\pm$1.66 
        & 51.23$\pm$0.25 
        & 45.61
        \\
        Moderate-DS 
        & 43.60$\pm$0.97 
        & 51.66$\pm$0.39 
        & 44.69$\pm$0.68 
        & 53.71$\pm$0.37 
        & 48.42
        \\
        {\bf $\gm$ Matching}
        & {\bf 45.41 $\pm$0.86}
        & {\bf 51.80 $\pm$1.01}
        & {\bf 49.78 $\pm$0.27}
        & {\bf 55.50 $\pm$0.31}
        & {\bf 50.62}
        \\
        \toprule
        & \multicolumn{2}{c}{\bf Tiny ImageNet (PGD Attack)} 
        & \multicolumn{2}{c}{\bf Tiny ImageNet (GS Attack)} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & 20\% 
        & 30\% 
        & 20\% 
        & 30\% 
        & {\bf Mean $\uparrow$} 
        \\
        \midrule
        Random 
        & 20.93$\pm$0.30 
        & 26.60$\pm$0.98 
        & 22.43$\pm$0.31 
        & 26.89$\pm$0.31 
        & 24.21
        \\
        Herding 
        & 21.61$\pm$0.36 
        & 25.95$\pm$0.19 
        & 23.04$\pm$0.28 
        & 27.39$\pm$0.14 
        & 24.50
        \\
        Forgetting 
        & 20.38$\pm$0.47 
        & 26.12$\pm$0.19 
        & 22.06$\pm$0.31 
        & 27.21$\pm$0.21 
        & 23.94
        \\
        GraNd-score 
        & 20.76$\pm$0.21 
        & 26.34$\pm$0.32 
        & 22.56$\pm$0.30 
        & 27.52$\pm$0.40 
        & 24.30
        \\
        EL2N-score 
        & 16.67$\pm$0.62 
        & 22.36$\pm$0.42 
        & 19.93$\pm$0.57 
        & 24.65$\pm$0.32 
        & 20.93
        \\
        Optimization-based 
        & 19.26$\pm$0.77 
        & 24.55$\pm$0.92 
        & 21.26$\pm$0.24 
        & 25.88$\pm$0.37 
        & 22.74
        \\
        Self-sup.-selection 
        & 19.23$\pm$0.46 
        & 23.92$\pm$0.51 
        & 19.70$\pm$0.20 
        & 24.73$\pm$0.39 
        & 21.90
        \\
        Moderate-DS 
        & 21.81$\pm$0.37 
        & 27.11$\pm$0.20 
        & 23.20$\pm$0.13 
        & 28.89$\pm$0.27 
        & 25.25
        \\
        {\bf $\gm$ Matching}
        & {\bf 25.98 $\pm$1.12}
        & {\bf 30.77 $\pm$0.25}
        & {\bf 29.71 $\pm$0.45}
        & {\bf 32.88 $\pm$0.73}
        & {\bf 29.84}
        \\
        \bottomrule
    \end{tabular}
    }
    \caption{
    \footnotesize
    {\bf \textsc{(Adversarial Attack) Image Classification:}} . Comparing (Test Accuracy) pruning methods under PGD and GS attacks. ResNet-50 is used both as proxy and for downstream classification.
    }
    \label{tab:main-A}
\end{table*}


==> tables/benchmark/tab-main-image-corr.tex <==
\begin{table*}[t]
\footnotesize
\centering
\resizebox{\textwidth}{!}
{
    \begin{tabular}{lccccccc}
        \toprule
        % \rowcolor{light-gray}
        % \multicolumn{8}{c}{{\bf CIFAR-100}}
        % \\
        % \midrule
        {\textbf{Method / Selection ratio}} 
        & \textbf{20\%} 
        & \textbf{30\%} 
        & \textbf{40\%}
        & \textbf{60\%}
        & \textbf{80\%}
        & \textbf{100\%}
        & \textbf{Mean $\uparrow$}
        % \\ 
        % \midrule
        % \multicolumn{8}{c}{{\bf No Corruption}}
        % \\
        % \midrule
        % Random              
        % & 50.26$\pm$3.24 
        % & 53.61$\pm$2.73 
        % & 64.32$\pm$1.77 
        % & 71.03$\pm$0.75 
        % & 74.12$\pm$0.56 
        % & 78.14$\pm$0.55 
        % & 62.67
        % \\ 
        % Herding               
        % & 48.39$\pm$1.42 
        % & 50.89$\pm$0.97 
        % & 62.99$\pm$0.61 
        % & 70.61$\pm$0.44 
        % & 74.21$\pm$0.49 
        % & 78.14$\pm$0.55 
        % & 61.42
        % \\ 
        % Forgetting            
        % & 35.57$\pm$1.40 
        % & 49.83$\pm$0.91 
        % & 59.65$\pm$2.50 
        % & \textbf{73.34$\pm$0.39} 
        % & \textbf{77.50$\pm$0.53} 
        % & 78.14$\pm$0.55 
        % & 59.18
        % \\ 
        % GraNd-score           
        % & 42.65$\pm$1.39 
        % & 53.14$\pm$1.28 
        % & 60.52$\pm$0.79 
        % & 69.70$\pm$0.68 
        % & 74.67$\pm$0.79 
        % & 78.14$\pm$0.55
        % & 60.14
        % \\ 
        % EL2N-score            
        % & 27.32$\pm$1.16 
        % & 41.98$\pm$0.54 
        % & 50.47$\pm$1.20 
        % & 69.23$\pm$1.00 
        % & 75.96$\pm$0.88 
        % & 78.14$\pm$0.55
        % & 52.99
        % \\ 
        % Optimization-based    
        % & 42.16$\pm$3.30 
        % & 53.19$\pm$2.14 
        % & 58.93$\pm$0.98 
        % & 68.93$\pm$0.70 
        % & 75.62$\pm$0.33 
        % & 78.14$\pm$0.55 
        % & 59.77
        % \\
        % Self-sup.-selection   
        % & 44.45$\pm$2.51
        % & 54.63$\pm$2.10 
        % & 62.91$\pm$1.20 
        % & 70.70$\pm$0.82 
        % & 75.29$\pm$0.45 
        % & 78.14$\pm$0.55 
        % & 61.60
        % \\ 
        % Moderate-DS
        % & 51.83$\pm$0.52
        % & 57.79$\pm$1.61
        % & 64.92$\pm$0.93
        % & 71.87$\pm$0.91 
        % & 75.44$\pm$0.40 
        % & 78.14$\pm$0.55 
        % & 64.37
        % \\ 
        % {\bf $\gm$ Matching}  
        % & {\bf 55.93$\pm$ 0.48}
        % & {\bf 63.08$\pm$ 0.57}
        % & {\bf 66.59$\pm$ 1.18} 
        % & 70.82$\pm$ 0.59
        % & 74.63$\pm$ 0.86
        % & 78.14$\pm$ 0.55  
        % & {\bf 66.01}
        % \\
        % \midrule
        % \multicolumn{8}{c}{{\bf 5\% Feature Corruption}}
        % \\
        % \midrule
        % Random              
        % & 43.14$\pm$3.04 
        % & 54.19$\pm$2.92 
        % & 64.21$\pm$2.39 
        % & 69.50$\pm$1.06 
        % & 72.90$\pm$0.52 
        % & 77.26$\pm$0.39 
        % & 60.79
        % \\ 
        % Herding               
        % & 42.50$\pm$1.27 
        % & 53.88$\pm$3.07 
        % & 60.54$\pm$0.94 
        % & 69.15$\pm$0.55 
        % & 73.47$\pm$0.89 
        % & 77.26$\pm$0.39 
        % & 59.81
        % \\ 
        % Forgetting            
        % & 32.42$\pm$0.74 
        % & 49.72$\pm$1.64 
        % & 54.84$\pm$2.20 
        % & 70.22$\pm$2.00 
        % & 75.19$\pm$0.40 
        % & 77.26$\pm$0.39 
        % & 56.48
        % \\ 
        % GraNd-score           
        % & 42.24$\pm$0.57 
        % & 53.48$\pm$0.76 
        % & 60.17$\pm$1.66 
        % & 69.16$\pm$0.81 
        % & 73.35$\pm$0.81 
        % & 77.26$\pm$0.39 
        % & 59.68
        % \\ 
        % EL2N-score            
        % & 26.13$\pm$1.75 
        % & 39.01$\pm$1.42 
        % & 49.89$\pm$1.87 
        % & 68.36$\pm$1.41 
        % & 73.10$\pm$0.36 
        % & 77.26$\pm$0.39 
        % & 51.30
        % \\ 
        % Optimization-based    
        % & 38.25$\pm$3.04 
        % & 50.88$\pm$6.07 
        % & 57.26$\pm$0.93 
        % & 68.02$\pm$0.39 
        % & 73.77$\pm$0.56 
        % & 77.26$\pm$0.39 
        % & 57.64
        % \\
        % Self-sup.-selection   
        % & 44.24$\pm$0.48 
        % & 55.99$\pm$1.21 
        % & 61.03$\pm$0.59 
        % & 69.96$\pm$1.07 
        % & 74.56$\pm$1.17 
        % & 77.26$\pm$0.39 
        % & 61.16
        % \\ 
        % Moderate-DS
        % & 46.78$\pm$1.90
        % & 57.36$\pm$1.22 
        % & 65.40$\pm$1.19
        % & 71.46$\pm$0.19 
        % & {\bf 75.64$\pm$0.61} 
        % & 77.26$\pm$0.39
        % & 63.33
        % \\
        % {\bf $\gm$ Matching}
        % & {\bf 49.50$\pm$0.72}
        % & {\bf 60.23$\pm$0.88}
        % & {\bf 66.25$\pm$0.51}
        % & {\bf 72.91$\pm$0.26}
        % & 75.10$\pm$0.29
        % & 77.26$\pm$0.39
        % & {\bf 64.80}
        % \\
        % \midrule
        % \multicolumn{8}{c}{{\bf 10\% Feature Corruption}}
        % \\
        % \midrule
        % Random              
        % & 43.27$\pm$3.01 
        % & 53.94$\pm$2.78 
        % & 62.17$\pm$1.29 
        % & 68.41$\pm$1.21 
        % & 73.50$\pm$0.73 
        % & 76.50$\pm$0.63 
        % & 60.26
        % \\ 
        % Herding               
        % & 44.34$\pm$1.07 
        % & 53.31$\pm$1.49 
        % & 60.13$\pm$0.38 
        % & 68.20$\pm$0.74 
        % & 74.34$\pm$1.07 
        % & 76.50$\pm$0.63 
        % & 60.06
        % \\ 
        % Forgetting            
        % & 30.43$\pm$0.70 
        % & 47.50$\pm$1.43 
        % & 53.16$\pm$0.44 
        % & 70.36$\pm$0.82 
        % & 75.11$\pm$0.71 
        % & 76.50$\pm$0.63 
        % & 55.31
        % \\ 
        % GraNd-score           
        % & 36.36$\pm$1.06 
        % & 52.26$\pm$0.66 
        % & 60.22$\pm$1.39 
        % & 68.96$\pm$0.62 
        % & 72.78$\pm$0.51 
        % & 76.50$\pm$0.63 
        % & 58.12
        % \\ 
        % EL2N-score            
        % & 21.75$\pm$1.56 
        % & 30.80$\pm$2.23 
        % & 41.06$\pm$1.23 
        % & 64.82$\pm$1.48 
        % & 73.47$\pm$1.30 
        % & 76.50$\pm$0.63 
        % & 46.38
        % \\ 
        % Optimization-based    
        % & 37.22$\pm$0.39 
        % & 48.92$\pm$1.38 
        % & 56.88$\pm$1.48 
        % & 67.33$\pm$2.15 
        % & 72.94$\pm$1.90 
        % & 76.50$\pm$0.63 
        % & 56.68
        % \\
        % Self-sup.-selection   
        % & 42.01$\pm$1.31 
        % & 54.47$\pm$1.19 
        % & 61.37$\pm$0.68 
        % & 68.52$\pm$1.24 
        % & 74.73$\pm$0.36 
        % & 76.50$\pm$0.63 
        % & 60.22
        % \\ 
        % Moderate-DS
        % & 47.02$\pm$0.66 
        % & 55.60$\pm$1.67 
        % & 62.18$\pm$1.86
        % & 71.83$\pm$0.78
        % & {\bf 75.66$\pm$0.66}
        % & 76.50$\pm$0.63
        % & 62.46
        % \\
        % {\bf $\gm$ Matching}
        % & {\bf 48.86$\pm$1.02}
        % & {\bf 60.15$\pm$0.43}
        % & {\bf 66.92$\pm$0.28}
        % & {\bf 72.03$\pm$0.38}
        % & 73.71$\pm$0.19
        % & 76.50$\pm$0.63
        % & {\bf 64.33}
        \\
        \midrule
        \multicolumn{8}{c}{{\bf CIFAR-100 with 20\% corrupted images}}
        \\
        \midrule
        Random              
        & 40.99$\pm$1.46 
        & 50.38$\pm$1.39 
        & 57.24$\pm$0.65 
        & 65.21$\pm$1.31 
        & 71.74$\pm$0.28 
        & 74.92$\pm$0.88 
        & 57.11
        \\ 
        Herding               
        & 44.42$\pm$0.46 
        & 53.57$\pm$0.31 
        & 60.72$\pm$1.78 
        & 69.09$\pm$1.73 
        & 73.08$\pm$0.98 
        & 74.92$\pm$0.88 
        & 60.18
        \\ 
        Forgetting            
        & 26.39$\pm$0.17 
        & 40.78$\pm$2.02 
        & 49.95$\pm$2.31 
        & 65.71$\pm$1.12 
        & 73.67$\pm$1.12 
        & 74.92$\pm$0.88 
        & 51.30
        \\ 
        GraNd-score           
        & 36.33$\pm$2.66 
        & 46.21$\pm$1.48 
        & 55.51$\pm$0.76 
        & 64.59$\pm$2.40 
        & 70.14$\pm$1.36 
        & 74.92$\pm$0.88 
        & 54.56
        \\ 
        EL2N-score            
        & 21.64$\pm$2.03 
        & 23.78$\pm$1.66 
        & 35.71$\pm$1.17 
        & 56.32$\pm$0.86 
        & 69.66$\pm$0.43 
        & 74.92$\pm$0.88 
        & 41.42
        \\ 
        Optimization-based    
        & 33.42$\pm$1.60 
        & 45.37$\pm$2.81 
        & 54.06$\pm$1.74 
        & 65.19$\pm$1.27 
        & 70.06$\pm$0.83 
        & 74.92$\pm$0.88 
        & 54.42
        \\
        Self-sup.-selection   
        & 42.61$\pm$2.44 
        & 54.04$\pm$1.90 
        & 59.51$\pm$1.22 
        & 68.97$\pm$0.96 
        & 72.33$\pm$0.20 
        & 74.92$\pm$0.88 
        & 60.01
        \\ 
        Moderate-DS
        & 42.98$\pm$0.87
        & 55.80$\pm$0.95
        & 61.84$\pm$1.96
        & 70.05$\pm$1.29 
        & 73.67$\pm$0.30
        & 74.92$\pm$0.88
        & 60.87
        \\
        {\bf $\gm$ Matching}
        & {\bf 47.12$\pm$0.64}
        & {\bf 59.17$\pm$0.92}
        & {\bf 63.45$\pm$0.34}
        & {\bf 71.70$\pm$0.60}
        & {\bf 74.60$\pm$1.03}
        & 74.92$\pm$0.88
        & {\bf 63.21}
        \\
        \midrule
        \multicolumn{8}{c}{{\bf Tiny ImageNet with 20 \% corrupted images}}
        \\
        \midrule
        Random              
        & 19.99$\pm$0.42 
        & 25.93$\pm$0.53 
        & 30.83$\pm$0.44 
        & 37.98$\pm$0.31 
        & 42.96$\pm$0.62 
        & 46.68$\pm$0.43 
        & 31.54
        \\ 
        Herding               
        & 19.46$\pm$0.14 
        & 24.47$\pm$0.33 
        & 29.72$\pm$0.39 
        & 37.50$\pm$0.59 
        & 42.28$\pm$0.30 
        & 46.68$\pm$0.43 
        & 30.86
        \\ 
        Forgetting            
        & 18.47$\pm$0.46 
        & 25.53$\pm$0.23 
        & 31.17$\pm$0.24 
        & 39.35$\pm$0.44 
        & 44.55$\pm$0.67 
        & 46.68$\pm$0.43 
        & 31.81
        \\ 
        GraNd-score           
        & 20.07$\pm$0.49 
        & 26.68$\pm$0.40 
        & 31.25$\pm$0.40 
        & 38.21$\pm$0.49 
        & 42.84$\pm$0.72 
        & 46.68$\pm$0.43 
        & 30.53
        \\ 
        EL2N-score            
        & 18.57$\pm$0.30 
        & 24.42$\pm$0.44 
        & 30.04$\pm$0.15 
        & 37.62$\pm$0.44 
        & 42.43$\pm$0.61 
        & 46.68$\pm$0.43 
        & 30.53
        \\ 
        Optimization-based    
        & 13.71$\pm$0.26 
        & 23.33$\pm$1.84 
        & 29.15$\pm$2.84 
        & 36.12$\pm$1.86 
        & 42.94$\pm$0.52 
        & 46.88$\pm$0.43 
        & 29.06
        \\
        Self-sup.-selection   
        & 20.22$\pm$0.23 
        & 26.90$\pm$0.50 
        & 31.93$\pm$0.49 
        & 39.74$\pm$0.52 
        & 44.27$\pm$0.10 
        & 46.68$\pm$0.43 
        & 32.61
        \\ 
        Moderate-DS
        & 23.27$\pm$0.33 
        & 29.06$\pm$0.36 
        & 33.48$\pm$0.11 
        & 40.07$\pm$0.36 
        & 44.73$\pm$0.39 
        & 46.68$\pm$0.43 
        & 34.12
        \\
        {\bf $\gm$ Matching}
        & {\bf 27.19$\pm$0.92}
        & {\bf 31.70$\pm$0.78}
        & {\bf 35.14$\pm$0.19}
        & {\bf 42.04$\pm$0.31}
        & {\bf 45.12$\pm$0.28} 
        & 46.68$\pm$0.43 
        & {\bf 36.24}
        \\
        \bottomrule
    \end{tabular}
}
    \caption{
    \footnotesize
    {\bf \textsc{(Feature Corruption) Image Classification:}} Experiments comparing pruning methods when 20\% of the images are corrupted. ResNet-50 is used for both proxy (data pruning) and downstream training.
    }
    \label{tab:main-C}
\end{table*}


==> tables/benchmark/tab-main-label-corr.tex <==
\begin{table*}
    \footnotesize
    \centering
    \resizebox{0.7\textwidth}{!}
{
    \begin{tabular}{lccccc}
        \toprule
        
        & \multicolumn{2}{c}{\bf CIFAR-100 (Label noise)} 
        & \multicolumn{2}{c}{\bf Tiny ImageNet (Label noise)} 
        & 
        \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio }
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf Mean $\uparrow$}
        \\
        \midrule
        \multicolumn{6}{c}{\bf 20\% Label Noise}
        \\
        \midrule
        Random 
        & 34.47$\pm$0.64 
        & 43.26$\pm$1.21 
        & 17.78$\pm$0.44 
        & 23.88$\pm$0.42 
        & 29.85
        \\
        Herding 
        & 42.29$\pm$1.75 
        & 50.52$\pm$3.38
        & 18.98$\pm$0.44 
        & 24.23$\pm$0.29 
        &  34.01
        \\
        Forgetting 
        & 36.53$\pm$1.11 
        & 45.78$\pm$1.04 
        & 13.20$\pm$0.38 
        & 21.79$\pm$0.43 
        & 29.33
        \\
        GraNd-score 
        & 31.72$\pm$0.67 
        & 42.80$\pm$0.30 
        & 18.28$\pm$0.32 
        & 23.72$\pm$0.18 
        & 28.05
        \\
        EL2N-score 
        & 29.82$\pm$1.19 
        & 33.62$\pm$2.35 
        & 13.93$\pm$0.69 
        & 18.57$\pm$0.31 
        & 23.99
        \\
        Optimization-based 
        & 32.79$\pm$0.62 
        & 41.80$\pm$1.14
        & 14.77$\pm$0.95 
        & 22.52$\pm$0.77 
        & 27.57
        \\
        Self-sup.-selection 
        & 31.08$\pm$0.78 
        & 41.87$\pm$0.63 
        & 15.10$\pm$0.73 
        & 21.01$\pm$0.36 
        & 27.27
        \\
        Moderate-DS 
        & 40.25$\pm$0.12 
        & 48.53$\pm$1.60 
        & 19.64$\pm$0.40 
        & 24.96$\pm$0.30
        & 31.33
        \\
        {\bf $\gm$ Matching}
        & {\bf 52.64$\pm$0.72}
        & {\bf 61.01$\pm$0.47}
        & {\bf 25.80$\pm$0.37} 
        & {\bf 31.71$\pm$0.24}
        & {\bf 42.79}
        \\
        \midrule
        \multicolumn{6}{c}{\bf 35\% Label Noise}
        \\
        \midrule
        Random 
        & 24.51$\pm$1.34 
        & 32.26$\pm$0.81 
        & 14.64$\pm$0.29 
        & 19.41$\pm$0.45 
        & 22.71
        \\
        Herding 
        & 29.42$\pm$1.54 
        & 37.50$\pm$2.12 
        & 15.14$\pm$0.45 
        & 20.19$\pm$0.45 
        & 25.56
        \\
        Forgetting 
        & 29.48$\pm$1.98 
        & 38.01$\pm$2.21 
        & 11.25$\pm$0.90 
        & 17.07$\pm$0.66 
        & 23.14
        \\
        GraNd-score 
        & 23.03$\pm$1.05 
        & 34.83$\pm$2.01 
        & 13.68$\pm$0.46 
        & 19.51$\pm$0.45 
        & 22.76
        \\
        EL2N-score 
        & 21.95$\pm$1.08 
        & 31.63$\pm$2.84 
        & 10.11$\pm$0.25 
        & 13.69$\pm$0.32 
        & 19.39
        \\
        Optimization-based 
        & 26.77$\pm$0.15 
        & 35.63$\pm$0.92 
        & 12.37$\pm$0.68 
        & 18.52$\pm$0.90 
        & 23.32
        \\
        Self-sup.-selection 
        & 23.12$\pm$1.47 
        & 34.85$\pm$0.68 
        & 11.23$\pm$0.32 
        & 17.76$\pm$0.69 
        & 22.64
        \\
        Moderate-DS 
        & 28.45$\pm$0.53 
        & 36.55$\pm$1.26 
        & 15.27$\pm$0.31 
        & 20.33$\pm$0.28 
        & 25.15
        \\
        {\bf $\gm$ Matching}
        & {\bf 43.33$\pm$ 1.02}
        & {\bf 58.41$\pm$ 0.68}
        & {\bf 23.14$\pm$ 0.92} 
        & {\bf 27.76$\pm$ 0.40}
        & {\bf 38.16}
        \\
        \bottomrule
    \end{tabular}
}
    \caption{
    \footnotesize
    {\bf \textsc{(Label Noise) Image Classification:}} Comparing (Test Accuracy) pruning methods on CIFAR-100 and TinyImageNet datasets, under 20\% and 35\% Symmetric Label Corruption, at 20\% and 30\% selection ratio. ResNet-50 is used both as proxy and for downstream classification.
    }
    \label{tab:main-N}
\end{table*}

==> tables/benchmark/tab-noisy-35.tex <==
\begin{table*}
    \footnotesize
    \centering
    \begin{tabular}{lccccc}
        \toprule
        
        & \multicolumn{2}{c}{\bf CIFAR-100 (Label noise)} 
        & \multicolumn{2}{c}{\bf Tiny ImageNet (Label noise)} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & 20\% 
        & 30\% 
        & 20\% 
        & 30\% 
        \\
        \midrule
        Random 
        & 24.51$\pm$1.34 
        & 32.26$\pm$0.81 
        & 14.64$\pm$0.29 
        & 19.41$\pm$0.45 

        \\
        Herding 
        & 29.42$\pm$1.54 
        & 37.50$\pm$2.12 
        & 15.14$\pm$0.45 
        & 20.19$\pm$0.45 

        \\
        Forgetting 
        & 29.48$\pm$1.98 
        & 38.01$\pm$2.21 
        & 11.25$\pm$0.90 
        & 17.07$\pm$0.66 

        \\
        GraNd-score 
        & 23.03$\pm$1.05 
        & 34.83$\pm$2.01 
        & 13.68$\pm$0.46 
        & 19.51$\pm$0.45 
        & 
        \\
        EL2N-score 
        & 21.95$\pm$1.08 
        & 31.63$\pm$2.84 
        & 10.11$\pm$0.25 
        & 13.69$\pm$0.32 
        & 
        \\
        Optimization-based 
        & 26.77$\pm$0.15 
        & 35.63$\pm$0.92 
        & 12.37$\pm$0.68 
        & 18.52$\pm$0.90 
        & 
        \\
        Self-sup.-selection 
        & 23.12$\pm$1.47 
        & 34.85$\pm$0.68 
        & 11.23$\pm$0.32 
        & 17.76$\pm$0.69 
        &
        \\
        Moderate-DS 
        & 28.45$\pm$0.53 
        & 36.55$\pm$1.26 
        & 15.27$\pm$0.31 
        & 20.33$\pm$0.28 
        & 
        \\
        {\bf $\gm$ Matching}
        & {\bf 43.33$\pm$ 1.02}
        & {\bf 58.41$\pm$ 0.68}
        & {\bf 23.14$\pm$ 0.92} 
        & {\bf 27.76$\pm$ 0.40}
        & 
        \\
        \bottomrule
    \end{tabular}
    \caption{35\% Label Noise}
    \label{tab:label-noise-0.35}
\end{table*}


==> tables/diffusion/corr-20-fid.tex <==
\begin{table}
\centering
\caption{
\footnotesize {\bf \textsc{Unconditional Image Generation (20\% Corruption)} }: FID Scores for training a Denoising Diffusion Probabilistic Model (DDPM) with data sampled by different methods across varying Subset Sizes. Bold values highlight the best performance at each subset size. Lower FID indicates better generative quality.
}
\label{tab:corr-20-fid_scores}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Sampling}} & \multicolumn{6}{c}{\textbf{Subset Size}} \\
\cmidrule(lr){2-7}
& \textbf{5\%} & \textbf{10\%} & \textbf{20\%} & \textbf{40\%} & \textbf{60\%} & \textbf{100\%} \\
\midrule
\textbf{Random}       
& 121.58
& 28.95
& 10.58
& 
&    
& 42.05
\\
\textbf{Easy}         
& \textcolor{gray}{\bf 102.72}
& 17.05
& 24.23
& 
&    
& 42.05
\\
\textbf{Hard}         
& 128.64
& 47.69
& 6.98
& 
&    
& 42.05
\\
\textbf{Moderate}     
& 114.61
& 14.86
& 11.73
& 
&    
& 42.05
\\
\textbf{Herding}      
& 129.10
& \textcolor{gray}{\bf 12.61}
& 13.96
& 
&    
& 42.05
\\
\textbf{GM Matching}  
& {\bf 87.31} 
& {\bf 12.52} 
& 14.91
& 
&    
& 42.05
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/diffusion/corr-30-fid.tex <==
\begin{table}
\centering
\caption{
\footnotesize {\bf \textsc{Unconditional Image Generation (30\% Corruption)}}: FID Scores for training a Denoising Diffusion Probabilistic Model (DDPM) with data sampled by different methods across varying Subset Sizes. Bold values highlight the best performance at each subset size. Lower FID indicates better generative quality.
}
\label{tab:corr-40-fid_scores}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Sampling}} & \multicolumn{6}{c}{\textbf{Subset Size}} \\
\cmidrule(lr){2-7}
& \textbf{5\%} & \textbf{10\%} & \textbf{20\%} & \textbf{40\%} & \textbf{60\%} & \textbf{100\%} \\
\midrule
\textbf{Random}       
& 121.97
& 19.02
& 5.26
& 
&    
& 65.55
\\
\textbf{Easy}         
& 90.06
& 18.81
& 19.67
& 
&    
& 65.55
\\
\textbf{Hard}         
& 124.31
& 25.82
& 22.59
& 
&    
& 65.55
\\
\textbf{Moderate}     
& 102.67    
& \textcolor{gray}{\bf 7.95}
& 20.13
& 
&    
& 65.55
\\
\textbf{Herding}      
& 125.67
& 10.20
& 14.68
& 
&    
& 65.55
\\
\textbf{GM Matching}  
& {\bf 73.57}
& {\bf 7.52}
& 12.30
& 
&    
& 65.55
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/diffusion/mnist-fid.tex <==
\begin{table}
\centering
\caption{
\footnotesize{\bf \textsc{Unconditional Image Generation}}: FID Scores for training a Denoising Diffusion Probabilistic Model (DDPM)~\citep{ho2020denoising} with data sampled by different methods across varying Subset Sizes and Corruption fractions from MNIST. Bold values highlight the best performance at each subset size and . Lower FID indicates better generative quality.
}
\label{tab:fid_scores}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Sampling}} & \multicolumn{5}{c}{\textbf{Subset Size}} \\
\cmidrule(lr){2-6}
& \textbf{5\%} & \textbf{10\%} & \textbf{20\%} & \textbf{40\%} & \textbf{100\%} \\
\midrule
\multicolumn{5}{c}{{\bf No Corruption}}
\\
\midrule
\textbf{Random}       
& 115.11
& {\bf 13.79}
& 10.93
& 3.68
& 0.48
\\
\textbf{Easy}         
& {\bf 95.13}
& 54.33
& 12.62
& 9.08
& 0.48
\\
\textbf{Hard}         
& 148.73
& 25.82
& 43.71
& 8.37
& 0.48
\\
\textbf{Moderate}     
& 119.40
& 28.87
& 14.72
& 5.26
& 0.48
\\
\textbf{Herding}      
& 120.21
& 52.18
& 18.76
& \textcolor{gray}{\bf 2.55}
& 0.48
\\
\textbf{GM Matching}  
& \textcolor{gray}{\bf 100.24}
& \textcolor{gray}{\bf 17.72}
& {\bf 5.26}
& {\bf 1.77}
& 0.48
\\
\midrule
\multicolumn{6}{c}{{\bf 20\% Corruption}}
\\
\midrule
\textbf{Random}       
& 121.58
& 89.02
& 60.58
& 52.76
& 42.05
\\
\textbf{Easy}         
& \textcolor{gray}{\bf 102.72}
& 87.05
& 34.23
& 21.06
& 42.05
\\
\textbf{Hard}         
& 128.64
& 87.69
& 56.98
& 48.17
& 42.05
\\
\textbf{Moderate}     
& 114.61
& 14.86
& 11.73
& 7.99
& 42.05
\\
\textbf{Herding}      
& 129.10
& 52.61
& 23.96
& 12.76
& 42.05
\\
\textbf{GM Matching}  
& {\bf 87.31} 
& {\bf 12.52} 
& 14.91
& 4.00
& 42.05
\\
\midrule
\multicolumn{6}{c}{{\bf 30\% Corruption}}
\\
\midrule
\textbf{Random}       
& 121.97
& 98.95
& 81.64
& 61.79
& 65.55
\\
\textbf{Easy}         
& 90.06
& 88.81
& 39.67
& 20.89
& 65.55
\\
\textbf{Hard}         
& 124.31
& 110.58
& 95.59
& 87.18
& 65.55
\\
\textbf{Moderate}     
& 102.67    
& \textcolor{gray}{\bf 17.95}
& 30.13
& 22.66
& 65.55
\\
\textbf{Herding}      
& 125.67
& 80.20
& 74.68
& 72.63
& 65.55
\\
\textbf{GM Matching}  
& {\bf 73.57}
& {\bf 7.52}
& {\bf 3.30}
& {\bf 2.45}
& 65.55
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

